Learning big logical rules by joining small rules

A major challenge in inductive logic programming is learning big rules. To address this challenge, we introduce an approach where we join small rules to learn big rules. We implement our approach in a constraint-driven system and use constraint solvers to efficiently join rules. Our experiments on many domains, including game playing and drug design, show that our approach can (i) learn rules with more than 100 literals, and (ii) drastically outperform existing approaches in terms of predictive accuracies.

==> B-samplecomplexity.tex <==

\section{Sample Complexity}


==> figures/A-background.tex <==

\section{Terminology}
\label{sec:bk}
% \subsection{Logic Programming}
We assume familiarity with logic programming \cite{lloyd:book} but restate some key relevant notation. A \emph{variable} is a string of characters starting with an uppercase letter. A \emph{predicate} symbol is a string of characters starting with a lowercase letter. The \emph{arity} $n$ of a function or predicate symbol is the number of arguments it takes. An \emph{atom} is a tuple $p(t_1, ..., t_n)$, where $p$ is a predicate of arity $n$ and $t_1$, ..., $t_n$ are terms, either variables or constants. An atom is \emph{ground} if it contains no variables. A \emph{literal} is an atom or the negation of an atom. A \emph{clause} is a set of literals. A \emph{clausal theory} is a set of clauses. A \emph{constraint} is a clause without a positive literal. A \emph{definite} clause is a clause with exactly one positive literal. 
A \emph{hypothesis} is a set of definite clauses with the least Herbrand semantics.
% A \emph{program} is a set of definite clauses. 
We use the term \emph{program} interchangeably with hypothesis, i.e. a \emph{hypothesis} is a \emph{program}. 
A \emph{substitution} $\theta = \{v_1 / t_1, ..., v_n/t_n \}$ is the simultaneous replacement of each variable $v_i$ by its corresponding term $t_i$. 
A clause $c_1$ \emph{subsumes} a clause $c_2$ if and only if there exists a substitution $\theta$ such that $c_1 \theta \subseteq c_2$. 
A program $h_1$ subsumes a program $h_2$, denoted $h_1 \preceq h_2$, if and only if $\forall c_2 \in h_2, \exists c_1 \in h_1$ such that $c_1$ subsumes $c_2$. A program $h_1$ is a \emph{specialisation} of a program $h_2$ if and only if $h_2 \preceq h_1$. A program $h_1$ is a \emph{generalisation} of a program $h_2$ if and only if $h_1 \preceq h_2$. 

% \subsection{Answer Set Programming}
% We also assume familiarity with answer set programming \cite{asp} but restate some key relevant notation \cite{ilasp}.
% A \emph{literal} can be either an atom $p$ or its \emph{default negation} $\text{not } p$ (often called \emph{negation by failure}). A normal rule is of the form $h \leftarrow b_1, ..., b_n, \text{not } c_1,... \text{not } c_m$. where $h$ is the \emph{head} of the rule, $b_1, ..., b_n, \text{not } c_1,... \text{not } c_m$ (collectively) is the \emph{body} of the rule, and all $h$, $b_i$, and $c_j$ are atoms. A \emph{constraint} is of the form $\leftarrow b_1, ..., b_n, \text{not } c_1,... \text{not } c_m.$ where the empty head means false. A \emph{choice rule} is an expression of the form $l\{h_1,...,h_m\}u \leftarrow b_1,...,b_n, \text{not } c_1,... \text{not } c_m$ where the head $l\{h_1,...,h_m\}u$ is called an \emph{aggregate}. In an aggregate, $l$ and $u$ are integers and $h_i$, for $1 \leq i \leq m$, are atoms. An \emph{answer set program} $P$ is a finite set of normal rules, constraints and choice rules. Given an answer set program $P$, the \emph{Herbrand base} of $P$, denoted
% as ${HB}_P$, is the set of all ground (variable free) atoms that can be formed from the predicates and constants that appear in $P$. When $P$ includes only normal rules, a set $A \in {HB}_P$ is an \emph{answer set} of $P$ iff it is the minimal model of the  \emph{reduct} $P^A$, which is the program constructed from the grounding of $P$ by first removing any rule whose body contains a literal $\text{not } c_i$ where $c_i \in A$, and then removing any defaultly negated literals in the remaining rules. An answer set $A$ satisfies a ground constraint $\leftarrow b_1, ..., b_n, \text{not } c_1,... \text{not } c_m.$ if it is not the case that $\{b_1, ..., b_n\} \in A$ and $A \cap \{c_1, ..., c_m\} = \emptyset$.

==> figures/A-encoding.tex <==
\section{Generate stage encoding}
\label{sec:encoding}
% \subsection{Generate} 
\label{generate}
Our encoding of the \emph{generate} stage is the same as \combo{} except we disallow splittable rules in hypotheses which are not recursive and do not contain predicate invention.
To do so, we add the following ASP program to the \emph{generate} encoding:
\begin{small}
\begin{verbatim}
:- not pi_or_rec, clause(C), splittable(C).

splittable(C) :-
     body_not_head(C,Var1),
     body_not_head(C,Var2),
     Var1 < Var2,
     not path(C,Var1,Var2).

path(C,Var1,Var2) :- path1(C,Var1,Var2).
path(C,Var1,Var2) :- 
    path1(C,Var1,Var3), 
    path(C,Var3,Var2).

path1(C,Var1,Var2) :-
     body_literal(C,_,_,Vars),
     var_member(Var1,Vars),
     var_member(Var2,Vars),
     Var1 < Var2,
     body_not_head(C,Var1),
     body_not_head(C,Var2).


%% we also disallow rules with multiple body 
literals when a body literal only has head variables
:- 
    not pi_or_rec, 
    body_literal(C,P1,_,Vars1), 
    body_literal(C,P2,_,Vars2), 
    (P1,Vars1) != (P2,Vars2), 
    head_only_vars(C,Vars1).

head_only_vars(C,Vars) :- 
    body_literal(C,_,_,Vars), 
    clause(C), 
    not has_body_var(C,Vars). 

has_body_var(C,Vars) :- 
    var_member(Var,Vars),
    body_not_head(C,Var).
    
body_not_head(C,V) :- 
    body_var(C,V), 
    not head_var(C,V).
\end{verbatim}
\end{small}

% \subsection{Specialiser}
% We describe the ASP encoding of the \emph{combine} stage. For each positive example, \name{} builds a unique example id. For instance, if the training set contains 6 positive examples, \name{} adds the following facts to the ASP encoding:
% \begin{verbatim}
% example(1).
% example(2).
% example(3).
% example(4).
% example(5).
% example(6).
% \end{verbatim}
% For each promising program, \name{} builds a unique rule id for each rule in that program. It generates a fact describing the rule size. It then generates facts describing the examples covered by this promising program. For instance, assume a promising program has two rules of size 2 and 3 respectively. The first rule is given the id 15, and the second already had been used in a previous program and had already been given the id 3. Assume this program covers the examples with id $\{1,2,4\}$. Then, \name{} adds the following facts to the ASP encoding:
% \begin{verbatim}
% size(15,2).
% covered(1) :- rule(15), rule(3).
% covered(2) :- rule(15), rule(3).
% covered(4) :- rule(15), rule(3).
% \end{verbatim}
% \name{} adds a choice rule which represents whether a rule is selected or not:
% \begin{verbatim}
% {rule(R)}:-size(R,_).
% \end{verbatim}
% \noindent
% \name{} adds a soft constraint to cover the maximum number of positive examples:\\
% \verb+:+$\sim$ \verb+ example(E), not covered(E). [1@2, (E,)]+\\
% Finally, \name{} adds a soft constraint to prefer models/programs with the smallest size:\\
% \verb+:+$\sim$ \verb+ rule(R),size(R,K). [K@1, (R,)]+\\
% If a combination has been found in a previous iteration, \name{} bounds the program size to ensure newly selected combinations have smaller sizes. For instance, assume \name{} has found a combination of size 10 in a previous iteration. Then, programs with a size greater than 10 cannot be optimal. \name{} adds the following constraint to restrict the search accordingly:
% \begin{verbatim}
% :- #sum{K,R : rule(R), size(R,K)} >= 10.
% \end{verbatim}
% Finally, \name{} uses the ASP system Clingo \cite{clingo} to try to find a model of the encoding.

==> figures/B-samplecomplexity.tex <==

\section{Sample Complexity}


==> figures/D-domains.tex <==
\section{Experiments}
\label{sec:exp}

\subsection{Experimental domains}
We describe the characteristics of the domains and tasks used in our experiments.
% in Tables \ref{tab:dataset} and \ref{tab:tasks}. 
Figure \ref{fig:sols} shows example solutions for some of the tasks.

% \begin{table}[ht!]
% \footnotesize
% \centering
% \begin{tabular}{@{}l|cccc@{}}
% % \toprule
% \textbf{Task} & \textbf{\# examples} & \textbf{\# relations} & \textbf{\# constants} & \textbf{\# facts}\\
% \midrule
% % \emph{imdb1} & 383 / 0 & 5 & 299 & 869 \\
% % \emph{imdb2} & 383 / 71442 & 5 & 299 & 869 \\
% % \emph{imdb3} & 69418 / 2438 & 5 & 299 & 869 \\
% \emph{attrition} & 672 & 12 & 65 & 163\\
% \emph{buttons} & 530 & 13 & 60 & 656 \\
% \emph{buttons-g} & 44 & 21 & 31 & 130 \\
% \emph{centipede} & 26 & 34 & 61 & 138 \\
% \emph{coins} & 2544 & 9 & 110 & 1101 \\
% \emph{coins-g} & 125 & 118 & 68 & 742 \\
% \emph{horseshoe} & 116 & 42 & 126 & 947\\
% \emph{md} & 54 & 12 & 13 & 29 \\
% \emph{rainbow} & 334 & 19 & 345 & 1332\\
% \emph{rps} & 464 & 6 & 64 & 405 \\
% \emph{sukoshi} & 296 & 14 & 151 & 1384 \\
% \midrule
% \emph{zendo1} & 100 & 16 & 1049 & 2270\\
% \emph{zendo2} & 100 & 16 & 1047 & 2184\\
% \emph{zendo3} & 100 & 16 & 1100 & 2320\\
% \emph{zendo4} & 100 & 16 & 987 & 2087\\
% \midrule
% \emph{imdb1} & 383 & 6 & 299 & 1330 \\
% \emph{imdb2} & 71825 & 6 & 299 & 1330 \\
% \emph{imdb3} & 121801 & 6 & 299 & 1330 \\
% \midrule
% \emph{pharma1} & 100 & 27 & 2600 & 72000\\
% \emph{pharma2} & 100 & 27 & 2600 & 72000\\
% \emph{pharma3} & 100 & 27 & 2600 & 72000\\
% \midrule
% \emph{strings1} & 600 & 29 & $\infty$ & $\infty$\\
% \emph{strings2} & 600 & 29 & $\infty$ & $\infty$\\
% \emph{strings3} & 600 & 29 & $\infty$ & $\infty$\\\midrule
% \emph{oned$\_$arc} & & 23 & & \\
% % \bottomrule
% \end{tabular}
% \caption{
% Experimental domain description.
% }

% % \ac{make clear the complexity ...}
% \label{tab:dataset}
% \end{table}

% \begin{table}[ht!]
% \footnotesize
% \centering
% \begin{tabular}{@{}l|cccc@{}}
% % \toprule
% \textbf{Task} & \textbf{\#rules} & \textbf{\#literals} & \textbf{max rule size} & \textbf{recursion}\\
% \midrule
% \emph{attrition} & 3 & 14 & 5& no\\
% \emph{buttons} & 10 & 61 & 7& no\\
% \emph{buttons-g} & 4 & 24 & 9 & no\\
% \emph{centipede} & 2 & 8 & 4& no\\
% \emph{coins} & 3 & 16 & 6 & no\\
% \emph{coins-g} & 4 & 21 & 6 & no \\
% \emph{horseshoe} & 3 & 21 & 9 & no\\
% \emph{md} & 2 & 11 & 6 & no\\
% \emph{rainbow} & 1 & 19 & 19 & no\\
% \emph{rps} & 4 & 25 & 7& no\\
% \emph{sukoshi} & 3 & 29 & 17 & no\\
% \midrule
% \emph{zendo1} & 1 & 7 & 7 & no\\
% \emph{zendo2} & 2 & 14 & 7 & no\\
% \emph{zendo3} & 3 & 20 & 7& no\\
% \emph{zendo4} & 4 & 23 & 7& no\\
% \midrule
% \emph{imdb1} & 1 & 5 & 5 & no\\
% \emph{imdb2} & 1 & 5 & 5 & no\\
% \emph{imdb3} & 2 & 10 & 5 & no\\
% \midrule
% \emph{pharma1} & 1 & 17 & 17 & no\\
% \emph{pharma2} & 1 & 19 & 19 & no\\
% \emph{pharma3} & 2 & 26 & 13 & no\\
% \midrule
% \emph{string1} & 9 & 29 & 5 & yes\\
% \emph{string2} & 13 & 43 & 7 & yes\\
% \emph{string3} & 10 & 30 & 3 & yes\\
% % \bottomrule
% \end{tabular}
% \caption{
% Statistics about the optimal solutions for each task.
% For instance, the optimal solution for \emph{buttons} has 10 rules and 61 literals and the largest rule has 7 literals.
% % \ac{@CH, add column for recursion?}
% % Note that these values are \emph{not} the bias settings.
% }

% \label{tab:tasks}
% \end{table}

\paragraph{IGGP.}
In \emph{inductive general game playing} (IGGP)  \cite{iggp} the task is to induce a hypothesis to explain game traces from the general game playing competition \cite{ggp}.
IGGP is notoriously difficult for machine learning approaches.
The currently best-performing system can only learn perfect solutions for 40\% of the tasks.
Moreover, although seemingly a toy problem, IGGP is representative of many real-world problems, such as inducing semantics of programming languages \cite{DBLP:conf/ilp/BarthaC19}. 
We use 11 tasks: \emph{minimal decay (md)}, \emph{buttons-next}, \emph{buttons-goal}, \emph{rock - paper - scissors (rps)}, \emph{coins-next}, \emph{coins-goal}, \emph{attrition}, \emph{centipede}, \emph{sukoshi}, \emph{rainbow}, and \emph{horseshoe}.

\paragraph{Zendo.} Zendo is an inductive game in which one player, the Master, creates a rule for structures made of pieces with varying attributes to follow. The other players, the Students, try to discover the rule by building and studying structures which are labelled by the Master as following or breaking the rule. The first student to correctly state the rule wins. We learn four increasingly complex rules for structures made of at most 5 pieces of varying color, size, orientation and position. 
Zendo is a challenging game that has attracted much interest in cognitive science \cite{zendo}.

\paragraph{IMDB.}
The real-world IMDB dataset \cite{mihalkova2007} includes relations between movies, actors, directors, movie genre, and gender. It has been created from the International Movie Database (IMDB.com) database. We learn the relation \emph{workedunder/2}, a more complex variant \emph{workedwithsamegender/2}, and the disjunction of the two.
This dataset is frequently used \cite{alps}.

\subsection{Experimental Setup}
We measure the mean and standard error of the predictive accuracy and learning time.
%We enforce a timeout of 600s per task.
%We repeat all the experiments 20 times.
%We measure the mean and standard error.
We use a 3.8 GHz 8-Core Intel Core i7 with 32GB of ram.
The systems use a single CPU.

% \textbf{Q1.}
% We compare the performance of \popper{} and \name{} on all the tasks.
% We use \popper{} 2.0.0 \cite{popper2}.

% \textbf{Q2.}
% We compare the performance of \popper{} and \name{} when varying the size of the hypothesis space.
% We vary the maximum size of a rule allowed in a hypothesis, ie the maximum number of literals in a rule.
% We focus on the \emph{md} task.

\subsection{Experimental Results}

% \subsubsection{Comparison against other ILP systems}

We compare \name{} against \combo{} and \ale{}, which we describe below.

% \paragraph{\popper{}.}
% One key experimental question is to see whether \dcc{} can 
\begin{description}
% \item[\popper{}] 
% We compare against \popper{} as \name{} directly improves on it.
% For instance, if given only a single positive example, \name{} is identical to \popper{}.
% In all the experiments, we give \name{} and \popper{} identical biases.
\item[\combo{}] \combo{} uses identical biases to \name{} so the comparison is direct, i.e. fair.

\item[\ale{}] \ale{} excels at learning many large non-recursive rules and should excel at the trains and IGGP tasks.
Although \ale{} can learn recursive programs, it struggles to do so.
\name{} and \ale{} use similar biases so the comparison can be considered reasonably fair.

\end{description}
\noindent
We also tried/considered other ILP systems.
We considered \ilasp{} \cite{ilasp}.
However, \ilasp{} builds on \ASPAL{} and first precomputes every possible rule in a hypothesis space, which is infeasible for our datasets.
In addition, \ilasp{} cannot learn Prolog programs so is unusable in the synthesis tasks.
For instance, it would require precomputing $10^{15}$ rules for the \emph{coins} task.
% For instance, on the trains tasks, \ilasp{} took 2 seconds to pre-compute rules with three body literals; 20 seconds for rules with four body literals; and 12 minutes for rules with five body literals.  \ch{still doable in 1h timeout}
% Since the simplest train task requires rules with six body literals, \ilasp{} is unusable.

\begin{figure*}
\centering
\footnotesize
\begin{lstlisting}[caption=zendo1\label{zendo1}]
zendo1(A):- piece(A,C),size(C,B),blue(C),small(B),contact(C,D),red(D).
\end{lstlisting}
\centering

\begin{lstlisting}[caption=zendo2\label{zendo2}]
zendo2(A):- piece(A,B),piece(A,D),piece(A,C),green(D),red(B),blue(C).
zendo2(A):- piece(A,D),piece(A,B),coord1(B,C),green(D),lhs(B),coord1(D,C).
\end{lstlisting}
\centering


\begin{lstlisting}[caption=zendo3\label{zendo3}]
zendo3(A):- piece(A,D),blue(D),coord1(D,B),piece(A,C),coord1(C,B),red(C).
zendo3(A):- piece(A,D),contact(D,C),rhs(D),size(C,B),large(B).
zendo3(A):- piece(A,B),upright(B),contact(B,D),blue(D),size(D,C),large(C).
\end{lstlisting}
\centering


\begin{lstlisting}[caption=zendo4\label{zendo4}]
zendo4(A):- piece(A,C),contact(C,B),strange(B),upright(C).
zendo4(A):- piece(A,D),contact(D,C),coord2(C,B),coord2(D,B).
zendo4(A):- piece(A,D),contact(D,C),size(C,B),red(D),medium(B).
zendo4(A):- piece(A,D),blue(D),lhs(D),piece(A,C),size(C,B),small(B).\end{lstlisting}
\centering

\begin{lstlisting}[caption=pharma1\label{pharma1}]
active(A):- atm(A,B),typec(B),bond1(B,C),typeo(C),atm(A,F),types(F),bonddu(F,G),typen(G),atm(A,D),
             typeh(D),bond2(D,E),typedu(E).
\end{lstlisting}
\centering

\begin{lstlisting}[caption=pharma2\label{pharma2}]
active(A):- atm(A,B),types(C),bonddu(C,B),atm(A,G),typeh(F),bond2(F,G),atm(A,E),typec(D),bond1(D,E).
active(A):- atm(A,B),typena(C),bondv(B,C),atm(A,N),typen(O),bondu(N,O),atm(A,F),typedu(G),bondar(G,F).
\end{lstlisting}
\centering

\begin{lstlisting}[caption=pharma3\label{pharma3}]
active(A):- atm(A,D),bond2(D,E),typeh(E),atm(A,C),bond1(C,B),typec(B).
active(A):- atm(A,B),typena(C),bondv(B,C),atm(A,N),typen(O),bondu(N,O).
\end{lstlisting}
\centering

\begin{lstlisting}[caption=string2\label{string2}]
f_1(A):- head(A,B),cm(B).
f_1(A):- tail(A,B),f_1(B).
f_2(A):- head(A,B),cd(B).
f_2(A):- tail(A,B),f_2(B).
f_3(A):- head(A,B),co(B).
f_3(A):- tail(A,B),f_3(B).
f_4(A):- head(A,B),cr(B).
f_4(A):- tail(A,B),f_4(B).
f_5(A):- head(A,B),cu(B).
f_5(A):- tail(A,B),f_5(B).
f(A):- f_1(A),f_2(A),f_3(A),f_4(A),f_5(A).
\end{lstlisting}
\centering

\begin{lstlisting}[caption=string3\label{string3}]
f_1(A):- head(A,B),cl(B).
f_1(A):- tail(A,B),f_1(B).
f_2(A):- head(A,B),ch(B).
f_2(A):- tail(A,B),f_2(B).
f_3(A):- head(A,B),cj(B).
f_3(A):- tail(A,B),f_3(B).
f_4(A):- head(A,B),cm(B).
f_4(A):- tail(A,B),f_4(B).
f(A):- f_1(A),f_2(A).
f(A):- f_3(A),f_4(A).
\end{lstlisting}
\caption{Example solutions.}
\label{fig:sols}
\end{figure*}

\begin{figure*}
\begin{lstlisting}[caption=minimal decay\label{minimaldecay}]
next_value(A,B):-c_player(D),c_pressButton(C),c5(B),does(A,D,C).
next_value(A,B):-c_player(C),my_true_value(A,E),does(A,C,D),my_succ(B,E),c_noop(D).
\end{lstlisting}

\begin{lstlisting}[caption=rainbow\label{rainbow}]
terminal(A):- mypos_r3(M),true_color(A,M,L),hue(L),mypos_r6(H),true_color(A,H,I),hue(I),mypos_r5(F),
            true_color(A,F,G),hue(G),mypos_r2(J),true_color(A,J,K),hue(K),mypos_r1(D),true_color(A,D,E),
            hue(E),mypos_r4(B),true_color(A,B,C),hue(C).
\end{lstlisting}

\begin{lstlisting}[caption=horseshoe\label{horseshoe}]
terminal(A):- int_20(B),true_step(A,B).
terminal(A):- mypos_b(E),mypos_c(G),true_cell(A,E,F),true_cell(A,G,F),mypos_d(D),
           true_cell(A,D,C),true_cell(A,B,C),adjacent(B,D).
terminal(A):- mypos_c(B),mypos_a(H),true_cell(A,H,I),mypos_b(J),true_cell(A,J,I),mypos_e(E),
           true_cell(A,B,D),true_cell(A,E,F),true_cell(A,G,F),adjacent(E,G),true_cell(A,C,D),adjacent(C,B).
\end{lstlisting}

\begin{lstlisting}[caption=buttons \label{buttons}]
next(A,B):-c_p(B),c_c(C),does(A,D,C),my_true(A,B),my_input(D,C).
next(A,B):-my_input(C,E),c_p(D),my_true(A,D),c_b(E),does(A,C,E),c_q(B).
next(A,B):-my_input(C,D),not_my_true(A,B),does(A,C,D),c_p(B),c_a(D).
next(A,B):-c_a(C),does(A,D,C),my_true(A,B),c_q(B),my_input(D,C).
next(A,B):-my_input(C,E),c_p(B),my_true(A,D),c_b(E),does(A,C,E),c_q(D).
next(A,B):-c_c(D),my_true(A,C),c_r(B),role(E),does(A,E,D),c_q(C).
next(A,B):-my_true(A,C),my_succ(C,B).
next(A,B):-my_input(C,D),does(A,C,D),my_true(A,B),c_r(B),c_b(D).
next(A,B):-my_input(C,D),does(A,C,D),my_true(A,B),c_r(B),c_a(D).
next(A,B):-my_true(A,E),c_c(C),does(A,D,C),c_q(B),c_r(E),my_input(D,C).
\end{lstlisting}
\begin{lstlisting}[caption=rps\label{rps}]
next_score(A,B,C):-does(A,B,E),different(G,B),my_true_score(A,B,F),beats(E,D),my_succ(F,C),does(A,G,D).
next_score(A,B,C):-different(G,B),beats(D,F),my_true_score(A,E,C),does(A,G,D),does(A,E,F).
next_score(A,B,C):-my_true_score(A,B,C),does(A,B,D),does(A,E,D),different(E,B).
\end{lstlisting}

\begin{lstlisting}[caption=coins\label{coins}]
next_cell(A,B,C):-does_jump(A,E,F,D),role(E),different(B,D),my_true_cell(A,B,C),different(F,B).
next_cell(A,B,C):-my_pos(E),role(D),c_zerocoins(C),does_jump(A,D,B,E).
next_cell(A,B,C):-role(D),does_jump(A,D,E,B),c_twocoins(C),different(B,E).
next_cell(A,B,C):-does_jump(A,F,E,D),role(F),my_succ(E,B),my_true_cell(A,B,C),different(E,D).
\end{lstlisting}

\begin{lstlisting}[caption=coins-goal\label{coins-goal}]
goal(A,B,C):- role(B),pos_5(D),my_true_step(A,D),score_100(C).
goal(A,B,C):- c_onecoin(E),my_pos(D),my_true_cell(A,D,E),score_0(C),role(B).
\end{lstlisting}
\caption{Example solutions.}
\end{figure*}






==> figures/E-results.tex <==

\section{Experimental results}

\subsection{Impact of the features}

\begin{table}[ht]
% \small
\centering
\footnotesize
\begin{tabular}{@{}l|ccc@{}}
% \toprule
\multirow{2}{*}{\textbf{Task}} & \multirow{2}{*}{\textbf{\combo{}}} & \textbf{with join} & \multirow{2}{*}{\textbf{\name{}}}\\
& & \textbf{splittable} & \\
\midrule
\emph{attrition} & 67 $\pm$ 0 & \textbf{75 $\pm$ 0} & 67 $\pm$ 0\\
\emph{buttons} & 91 $\pm$ 0 & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{buttons-g} & \textbf{100 $\pm$ 0} & 90 $\pm$ 0 & 98 $\pm$ 2\\
\emph{centipede} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{coins} & 62 $\pm$ 0 & \textbf{100 $\pm$ 0} & 80 $\pm$ 0\\
\emph{coins-g} & \textbf{97 $\pm$ 0} & \textbf{97 $\pm$ 0} & \textbf{97 $\pm$ 0}\\
\emph{horseshoe} & 67 $\pm$ 0 & 69 $\pm$ 8 & \textbf{100 $\pm$ 0}\\
\emph{md} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{rainbow} & 50 $\pm$ 0 & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{rps} & 50 $\pm$ 0 & 82 $\pm$ 0 & \textbf{100 $\pm$ 0}\\
\emph{sukoshi} & 50 $\pm$ 0 & 50 $\pm$ 0 & \textbf{99 $\pm$ 0}\\\midrule
\emph{imdb1} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{imdb2} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{imdb3} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\\midrule
\emph{pharma1} & 50 $\pm$ 0 & 56 $\pm$ 2 & \textbf{57 $\pm$ 1}\\
\emph{pharma2} & 50 $\pm$ 0 & \textbf{99 $\pm$ 1} & 98 $\pm$ 1\\
\emph{pharma3} & 50 $\pm$ 0 & \textbf{97 $\pm$ 1} & 96 $\pm$ 1\\\midrule
\emph{zendo1} & 94 $\pm$ 3 & \textbf{99 $\pm$ 0} & \textbf{99 $\pm$ 1}\\
\emph{zendo2} & 70 $\pm$ 1 & 92 $\pm$ 1 & \textbf{93 $\pm$ 1}\\
\emph{zendo3} & 79 $\pm$ 1 & 79 $\pm$ 1 & \textbf{80 $\pm$ 1}\\
\emph{zendo4} & 93 $\pm$ 1 & \textbf{99 $\pm$ 1} & \textbf{99 $\pm$ 1}\\\midrule
\emph{string1} & 50 $\pm$ 0 & \textbf{53 $\pm$ 1} & \textbf{53 $\pm$ 1}\\
\emph{string2} & 50 $\pm$ 0 & \textbf{53 $\pm$ 1} & \textbf{53 $\pm$ 1}\\
\emph{string3} & 50 $\pm$ 0 & 51 $\pm$ 2 & \textbf{100 $\pm$ 0}\\\midrule
\emph{denoising$\_$1c} & 52 $\pm$ 2 & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{denoising$\_$mc} & 60 $\pm$ 10 & \textbf{99 $\pm$ 1} & \textbf{99 $\pm$ 1}\\
\emph{fill} & 52 $\pm$ 2 & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{flip} & 50 $\pm$ 0 & \textbf{85 $\pm$ 9} & \textbf{85 $\pm$ 9}\\
\emph{hollow} & \textbf{55 $\pm$ 5} & \textbf{55 $\pm$ 5} & \textbf{55 $\pm$ 5}\\
\emph{mirror} & 57 $\pm$ 1 & \textbf{61 $\pm$ 4} & \textbf{61 $\pm$ 4}\\
\emph{move$\_$1p} & 50 $\pm$ 0 & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{move$\_$2p} & 50 $\pm$ 0 & 80 $\pm$ 8 & \textbf{88 $\pm$ 4}\\
\emph{move$\_$2p$\_$dp} & 55 $\pm$ 2 & 87 $\pm$ 8 & \textbf{88 $\pm$ 9}\\
\emph{move$\_$3p} & 50 $\pm$ 0 & 62 $\pm$ 9 & \textbf{64 $\pm$ 9}\\
\emph{move$\_$dp} & 55 $\pm$ 2 & \textbf{65 $\pm$ 6} & 62 $\pm$ 3\\
\emph{padded$\_$fill} & 52 $\pm$ 2 & \textbf{66 $\pm$ 3} & \textbf{66 $\pm$ 3}\\
\emph{pcopy$\_$1c} & 50 $\pm$ 0 & \textbf{86 $\pm$ 9} & 84 $\pm$ 9\\
\emph{pcopy$\_$mc} & 68 $\pm$ 6 & \textbf{97 $\pm$ 2} & \textbf{97 $\pm$ 2}\\
\emph{recolor$\_$cmp} & 51 $\pm$ 1 & \textbf{55 $\pm$ 4} & \textbf{55 $\pm$ 4}\\
\emph{recolor$\_$cnt} & 50 $\pm$ 0 & \textbf{51 $\pm$ 1} & \textbf{51 $\pm$ 1}\\
\emph{recolor$\_$oe} & 50 $\pm$ 0 & \textbf{52 $\pm$ 2} & \textbf{52 $\pm$ 2}\\
\emph{scale$\_$dp} & 61 $\pm$ 8 & 96 $\pm$ 2 & \textbf{97 $\pm$ 2}\\
\end{tabular}
\caption{
Predictive accuracies with a 60s timeout. We round accuracies to integer values. The error is standard error.
}
\label{tab:accuracies_60}
\end{table}

\begin{table}[ht]
% \small
\centering
\footnotesize
\begin{tabular}{@{}l|ccc@{}}
% \toprule
\multirow{2}{*}{\textbf{Task}} & \multirow{2}{*}{\textbf{\combo{}}} & \textbf{with join} & \multirow{2}{*}{\textbf{\name{}}}\\
& & \textbf{splittable} & \\
\midrule
\emph{attrition} & 67 $\pm$ 0 & \textbf{73 $\pm$ 2} & 67 $\pm$ 0\\
\emph{buttons} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{buttons-g} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0} & 96 $\pm$ 2\\
\emph{centipede} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{coins} & 85 $\pm$ 9 & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{coins-g} & \textbf{97 $\pm$ 0} & \textbf{97 $\pm$ 0} & \textbf{97 $\pm$ 0}\\
\emph{horseshoe} & 67 $\pm$ 0 & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{md} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{rainbow} & 52 $\pm$ 0 & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{rps} & 77 $\pm$ 0 & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{sukoshi} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\\midrule
\emph{imdb1} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{imdb2} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{imdb3} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\\midrule
\emph{pharma1} & 50 $\pm$ 0 & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{pharma2} & 50 $\pm$ 0 & \textbf{98 $\pm$ 1} & 97 $\pm$ 1\\
\emph{pharma3} & 58 $\pm$ 5 & \textbf{96 $\pm$ 1} & \textbf{96 $\pm$ 1}\\\midrule
\emph{zendo1} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{zendo2} & 72 $\pm$ 1 & 93 $\pm$ 1 & \textbf{100 $\pm$ 0}\\
\emph{zendo3} & \textbf{79 $\pm$ 1} & 78 $\pm$ 1 & \textbf{79 $\pm$ 1}\\
\emph{zendo4} & 92 $\pm$ 1 & \textbf{98 $\pm$ 1} & \textbf{98 $\pm$ 1}\\\midrule
\emph{string1} & 50 $\pm$ 0 & 56 $\pm$ 1 & \textbf{100 $\pm$ 0}\\
\emph{string2} & 51 $\pm$ 0 & 56 $\pm$ 1 & \textbf{100 $\pm$ 0}\\
\emph{string3} & 49 $\pm$ 0 & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\\midrule
\emph{denoising$\_$1c} & 52 $\pm$ 2 & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{denoising$\_$mc} & 60 $\pm$ 10 & \textbf{99 $\pm$ 1} & 97 $\pm$ 2\\
\emph{fill} & 59 $\pm$ 5 & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{flip} & 58 $\pm$ 8 & 94 $\pm$ 4 & \textbf{96 $\pm$ 4}\\
\emph{hollow} & 55 $\pm$ 5 & 85 $\pm$ 10 & \textbf{90 $\pm$ 6}\\
\emph{mirror} & 57 $\pm$ 1 & \textbf{78 $\pm$ 10} & 70 $\pm$ 3\\
\emph{move$\_$1p} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{move$\_$2p} & 50 $\pm$ 0 & 81 $\pm$ 9 & \textbf{91 $\pm$ 9}\\
\emph{move$\_$2p$\_$dp} & 55 $\pm$ 2 & 89 $\pm$ 9 & \textbf{100 $\pm$ 0}\\
\emph{move$\_$3p} & 50 $\pm$ 0 & 64 $\pm$ 9 & \textbf{85 $\pm$ 3}\\
\emph{move$\_$dp} & 55 $\pm$ 2 & 58 $\pm$ 2 & \textbf{83 $\pm$ 5}\\
\emph{padded$\_$fill} & 52 $\pm$ 2 & 66 $\pm$ 3 & \textbf{86 $\pm$ 5}\\
\emph{pcopy$\_$1c} & 50 $\pm$ 0 & 84 $\pm$ 9 & \textbf{92 $\pm$ 6}\\
\emph{pcopy$\_$mc} & 68 $\pm$ 6 & \textbf{97 $\pm$ 2} & 95 $\pm$ 3\\
\emph{recolor$\_$cmp} & 51 $\pm$ 1 & 58 $\pm$ 5 & \textbf{68 $\pm$ 5}\\
\emph{recolor$\_$cnt} & 50 $\pm$ 0 & 61 $\pm$ 7 & \textbf{80 $\pm$ 4}\\
\emph{recolor$\_$oe} & 50 $\pm$ 0 & 69 $\pm$ 8 & \textbf{75 $\pm$ 7}\\
\emph{scale$\_$dp} & 61 $\pm$ 8 & 96 $\pm$ 2 & \textbf{100 $\pm$ 0}\\
\end{tabular}
\caption{
Predictive accuracies with a 600s timeout. We round accuracies to integer values. The error is standard error.
}
\label{tab:accuracies_600}
\end{table}


\subsection{Comparison against other systems}


\begin{table}[ht]
% \small
\centering
\footnotesize
\begin{tabular}{@{}l|cccc@{}}
\textbf{Task} & \textbf{\ale} & \textbf{\combo} & \textbf{\name}\\ \midrule
\emph{attrition} & 50 $\pm$ 0 & \textbf{67 $\pm$ 0} & \textbf{67 $\pm$ 0}\\
\emph{buttons} & 50 $\pm$ 0 & 91 $\pm$ 0 & \textbf{100 $\pm$ 0}\\
\emph{buttons-g} & 50 $\pm$ 0 & \textbf{100 $\pm$ 0} & 98 $\pm$ 2\\
\emph{centipede} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{coins} & 50 $\pm$ 0 & 62 $\pm$ 0 & \textbf{80 $\pm$ 0}\\
\emph{coins-g} & \textbf{100 $\pm$ 0} & 97 $\pm$ 0 & 97 $\pm$ 0\\
\emph{horseshoe} & 50 $\pm$ 0 & 67 $\pm$ 0 & \textbf{100 $\pm$ 0}\\
\emph{md} & 97 $\pm$ 0 & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{rainbow} & 50 $\pm$ 0 & 50 $\pm$ 0 & \textbf{100 $\pm$ 0}\\
\emph{rps} & 50 $\pm$ 0 & 50 $\pm$ 0 & \textbf{100 $\pm$ 0}\\
\emph{sukoshi} & 50 $\pm$ 0 & 50 $\pm$ 0 & \textbf{99 $\pm$ 0}\\\midrule
\emph{imdb1} & 60 $\pm$ 10 & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{imdb2} & 50 $\pm$ 0 & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{imdb3} & 50 $\pm$ 0 & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\\midrule
\emph{pharma1} & 50 $\pm$ 0 & 50 $\pm$ 0 & \textbf{57 $\pm$ 1}\\
\emph{pharma2} & 50 $\pm$ 0 & 50 $\pm$ 0 & \textbf{98 $\pm$ 1}\\
\emph{pharma3} & 50 $\pm$ 0 & 50 $\pm$ 0 & \textbf{96 $\pm$ 1}\\\midrule
\emph{zendo1} & \textbf{100 $\pm$ 0} & 94 $\pm$ 3 & 99 $\pm$ 1\\
\emph{zendo2} & \textbf{100 $\pm$ 0} & 70 $\pm$ 1 & 93 $\pm$ 1\\
\emph{zendo3} & \textbf{99 $\pm$ 0} & 79 $\pm$ 1 & 80 $\pm$ 1\\
\emph{zendo4} & \textbf{99 $\pm$ 1} & 93 $\pm$ 1 & \textbf{99 $\pm$ 1}\\\midrule
\emph{string1} & 50 $\pm$ 0 & 50 $\pm$ 0 & \textbf{53 $\pm$ 1}\\
\emph{string2} & 50 $\pm$ 0 & 50 $\pm$ 0 & \textbf{53 $\pm$ 1}\\
\emph{string3} & 50 $\pm$ 0 & 50 $\pm$ 0 & \textbf{100 $\pm$ 0}\\\midrule
\emph{denoising$\_$1c} & 50 $\pm$ 0 & 52 $\pm$ 2 & \textbf{100 $\pm$ 0}\\
\emph{denoising$\_$mc} & 50 $\pm$ 0 & 60 $\pm$ 10 & \textbf{99 $\pm$ 1}\\
\emph{fill} & 50 $\pm$ 0 & 52 $\pm$ 2 & \textbf{100 $\pm$ 0}\\
\emph{flip} & 50 $\pm$ 0 & 50 $\pm$ 0 & \textbf{85 $\pm$ 9}\\
\emph{hollow} & 50 $\pm$ 0 & \textbf{55 $\pm$ 5} & \textbf{55 $\pm$ 5}\\
\emph{mirror} & 50 $\pm$ 0 & 57 $\pm$ 1 & \textbf{61 $\pm$ 4}\\
\emph{move$\_$1p} & 50 $\pm$ 0 & 50 $\pm$ 0 & \textbf{100 $\pm$ 0}\\
\emph{move$\_$2p} & 50 $\pm$ 0 & 50 $\pm$ 0 & \textbf{88 $\pm$ 4}\\
\emph{move$\_$2p$\_$dp} & 50 $\pm$ 0 & 55 $\pm$ 2 & \textbf{88 $\pm$ 9}\\
\emph{move$\_$3p} & 50 $\pm$ 0 & 50 $\pm$ 0 & \textbf{64 $\pm$ 9}\\
\emph{move$\_$dp} & 50 $\pm$ 0 & 55 $\pm$ 2 & \textbf{62 $\pm$ 3}\\
\emph{padded$\_$fill} & 50 $\pm$ 0 & 52 $\pm$ 2 & \textbf{66 $\pm$ 3}\\
\emph{pcopy$\_$1c} & 50 $\pm$ 0 & 50 $\pm$ 0 & \textbf{84 $\pm$ 9}\\
\emph{pcopy$\_$mc} & 50 $\pm$ 0 & 68 $\pm$ 6 & \textbf{97 $\pm$ 2}\\
\emph{recolor$\_$cmp} & 50 $\pm$ 0 & 51 $\pm$ 1 & \textbf{55 $\pm$ 4}\\
\emph{recolor$\_$cnt} & 50 $\pm$ 0 & 50 $\pm$ 0 & \textbf{51 $\pm$ 1}\\
\emph{recolor$\_$oe} & 50 $\pm$ 0 & 50 $\pm$ 0 & \textbf{52 $\pm$ 2}\\
\emph{scale$\_$dp} & 50 $\pm$ 0 & 61 $\pm$ 8 & \textbf{97 $\pm$ 2}\\
\end{tabular}
\caption{
Predictive accuracies with a 60s timeout. We round accuracies to integer values. The error is standard error.
% The tasks below the double line require negation while the one above do not.
%\ac{captions should not be centered} 
}
\label{tab:acc_sota_60}
\end{table}

\begin{table}[ht]
% \small
\centering
\footnotesize
\begin{tabular}{@{}l|cccc@{}}
% \toprule
\textbf{Task} & \textbf{\ale} & \textbf{\combo} & \textbf{\name}\\ \midrule
\emph{attrition} & 50 $\pm$ 0 & \textbf{67 $\pm$ 0} & \textbf{67 $\pm$ 0}\\
\emph{buttons} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{buttons-g} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0} & 96 $\pm$ 2\\
\emph{centipede} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{coins} & 50 $\pm$ 0 & 85 $\pm$ 9 & \textbf{100 $\pm$ 0}\\
\emph{coins-g} & \textbf{100 $\pm$ 0} & 97 $\pm$ 0 & 97 $\pm$ 0\\
\emph{horseshoe} & 65 $\pm$ 0 & 67 $\pm$ 0 & \textbf{100 $\pm$ 0}\\
\emph{md} & 97 $\pm$ 0 & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{rainbow} & 50 $\pm$ 0 & 52 $\pm$ 0 & \textbf{100 $\pm$ 0}\\
\emph{rps} & \textbf{100 $\pm$ 0} & 77 $\pm$ 0 & \textbf{100 $\pm$ 0}\\
\emph{sukoshi} & 50 $\pm$ 0 & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\\midrule
\emph{imdb1} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{imdb2} & 50 $\pm$ 0 & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{imdb3} & 50 $\pm$ 0 & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\\midrule
\emph{pharma1} & 50 $\pm$ 0 & 50 $\pm$ 0 & \textbf{100 $\pm$ 0}\\
\emph{pharma2} & 50 $\pm$ 0 & 50 $\pm$ 0 & \textbf{97 $\pm$ 1}\\
\emph{pharma3} & 50 $\pm$ 0 & 58 $\pm$ 5 & \textbf{96 $\pm$ 1}\\\midrule
\emph{zendo1} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{zendo2} & \textbf{100 $\pm$ 0} & 72 $\pm$ 1 & \textbf{100 $\pm$ 0}\\
\emph{zendo3} & \textbf{100 $\pm$ 0} & 79 $\pm$ 1 & 79 $\pm$ 1\\
\emph{zendo4} & \textbf{99 $\pm$ 0} & 92 $\pm$ 1 & 98 $\pm$ 1\\\midrule
\emph{string1} & 50 $\pm$ 0 & 50 $\pm$ 0 & \textbf{100 $\pm$ 0}\\
\emph{string2} & 50 $\pm$ 0 & 51 $\pm$ 0 & \textbf{100 $\pm$ 0}\\
\emph{string3} & 50 $\pm$ 0 & 49 $\pm$ 0 & \textbf{100 $\pm$ 0}\\\midrule
\emph{denoising$\_$1c} & 50 $\pm$ 0 & 52 $\pm$ 2 & \textbf{100 $\pm$ 0}\\
\emph{denoising$\_$mc} & 50 $\pm$ 0 & 60 $\pm$ 10 & \textbf{97 $\pm$ 2}\\
\emph{fill} & 50 $\pm$ 0 & 59 $\pm$ 5 & \textbf{100 $\pm$ 0}\\
\emph{flip} & 50 $\pm$ 0 & 58 $\pm$ 8 & \textbf{96 $\pm$ 4}\\
\emph{hollow} & 55 $\pm$ 5 & 55 $\pm$ 5 & \textbf{90 $\pm$ 6}\\
\emph{mirror} & 60 $\pm$ 8 & 57 $\pm$ 1 & \textbf{70 $\pm$ 3}\\
\emph{move$\_$1p} & 50 $\pm$ 0 & \textbf{100 $\pm$ 0} & \textbf{100 $\pm$ 0}\\
\emph{move$\_$2p} & 50 $\pm$ 0 & 50 $\pm$ 0 & \textbf{91 $\pm$ 9}\\
\emph{move$\_$2p$\_$dp} & 50 $\pm$ 0 & 55 $\pm$ 2 & \textbf{100 $\pm$ 0}\\
\emph{move$\_$3p} & 50 $\pm$ 0 & 50 $\pm$ 0 & \textbf{85 $\pm$ 3}\\
\emph{move$\_$dp} & 50 $\pm$ 0 & 55 $\pm$ 2 & \textbf{83 $\pm$ 5}\\
\emph{padded$\_$fill} & 50 $\pm$ 0 & 52 $\pm$ 2 & \textbf{86 $\pm$ 5}\\
\emph{pcopy$\_$1c} & 50 $\pm$ 0 & 50 $\pm$ 0 & \textbf{92 $\pm$ 6}\\
\emph{pcopy$\_$mc} & 50 $\pm$ 0 & 68 $\pm$ 6 & \textbf{95 $\pm$ 3}\\
\emph{recolor$\_$cmp} & 50 $\pm$ 0 & 51 $\pm$ 1 & \textbf{68 $\pm$ 5}\\
\emph{recolor$\_$cnt} & 56 $\pm$ 6 & 50 $\pm$ 0 & \textbf{80 $\pm$ 4}\\
\emph{recolor$\_$oe} & 50 $\pm$ 0 & 50 $\pm$ 0 & \textbf{75 $\pm$ 7}\\
\emph{scale$\_$dp} & 50 $\pm$ 0 & 61 $\pm$ 8 & \textbf{100 $\pm$ 0}\\
\end{tabular}
\caption{
Predictive accuracies with a 600s timeout. We round accuracies to integer values. The error is standard error.
% The tasks below the double line require negation while the one above do not.
%\ac{captions should not be centered} 
}
\label{tab:acc_sota_600}
\end{table}






==> figures/correctness.tex <==
\section{\name{} Correctness}
\label{sec:proof}
We show the correctness of \name{}.
In the rest of this section, we consider a LFF input tuple $(E, B, \mathcal{H}, C)$ with $E=(E^+, E^-)$. We assume that a solution always exists:
\begin{assumption}[\textbf{Existence of a solution}] \label{existencesol}We assume there exists a solution $h \in \mathcal{H}_{C}$.
\end{assumption}
\noindent
For terseness, in the rest of this section we always assume Assumption \ref{existencesol} and, therefore, avoid repeatedly saying ``if a solution exists''.

We follow LFF \cite{popper} and assume the background knowledge does not depend on any hypothesis:
\begin{assumption}[\textbf{Background knowledge independence}] \label{independentbk}We assume that no predicate symbol in the body of a rule in the background knowledge appears in the head of a rule in a hypothesis. 
\end{assumption}
% In other words, we assume that the BK does not depend on any hypothesis.
\noindent
For instance, given the following background knowledge we disallow learning hypotheses for the target relations \emph{famous} or \emph{friend}:
\begin{center}
\begin{tabular}{l}
\emph{happy(A) $\leftarrow$ friend(A,B), famous(B)}\\
\end{tabular}
\end{center}
% \ch{do we need this?}

\noindent
As with \combo{} \cite{combo}, \name{} is correct when the hypothesis space only contains decidable programs (such as Datalog programs), i.e. when every program is guaranteed to terminate:
\begin{assumption}[\textbf{Decidable programs}]\label{decidable}
We assume the hypothesis space only contains decidable programs.
\end{assumption}
% which also holds for \popper{} \cite{popper}, 
\noindent
When the hypothesis space contains arbitrary definite programs, the results do not hold because, due to their Turing completeness, checking entailment of an arbitrary definite program is semi-decidable \cite{tarnlund:hornclause}, i.e. testing a program might never terminate.
% \ch{perhaps number the assumptions to refer back to them}

\name{} follows a generate, test, join, combine, and constrain loop. We show the correctness of each of these steps in turn.
% We follow the proof of the correctness of \combo{} \cite{combo} and we prove the correctness of \name{} in three steps. 
% We first assume that there is no constrain stage, i.e. \name{} does not apply constraints.
% With this assumption, we show that the generate, test, join and combine stages return an optimal solution. 
% We then show that the constrain stage is optimally sound in that it never prunes optimal solutions from the hypothesis space.
We finally use these results to prove the correctness of \name{} i.e. that \name{} returns an optimal solution.

\subsection{Preliminaries}
We introduce definitions used throughout this section.
We define a splittable rule:
\begin{definition}[\textbf{Splittable rule}]
A rule is splittable if its body literals can be partitioned into two non-empty sets such that the body-only variables (a variable in the body of a rule but not the head) in the literals of one set are disjoint from the body-only variables in the literals of the other set.
A rule is non-splittable if it is not splittable.
\label{def:splittablerule}
\end{definition}

\noindent
We define a splittable program:
\begin{definition}
[\textbf{Splittable program}]
A program is \emph{splittable} if and only if it has exactly one rule and this rule is splittable.
A program is non-splittable when it is not splittable.
\label{def:splittable}
\end{definition}

\noindent
The least Herbrand model $M(P)$ of the logic program $P$ is the set of all ground atomic logical consequences of $P$,
The least Herbrand model $M_{B}(P) = M(P \cup B)$ of $P$ given the logic program $B$ is the the set of all ground atomic logical consequences of $P \cup B$. 
In the following, we assume a program $B$ denoting background knowledge and concisely note $M_{B}(P)$ as $M(P)$.



% \ac{@CH, I would move these definitions just before they are used as I would skip this section when reading a paper.}


We define a conjunction:
\begin{definition}[\textbf{Conjunction}]
A conjunction is a set of programs with the same head literal. 
The logical consequences of a conjunction $c$ is the intersection of the logical consequences of the programs in it: $M(c) = \cap_{p \in c} M(p)$. 
The cost of a conjunction $c$ is the sum of the cost of the programs in it: $cost(c) = \sum_{p\in c} cost(p)$.
\label{conjunction}
\end{definition}

\noindent
Conjunctions only preserve the semantics with respect to their head predicate symbols.
We, therefore, reason about the least Herbrand model restricted to a predicate symbol:
\begin{definition}[\textbf{Restricted least Herbrand model}]
Let $P$ be a logic program and $f$ be a predicate symbol. 
Then the least Herbrand model of $P$ restricted to $f$ is $M(P,f) = \{ a \in M(P) \,|\, \text{the predicate symbol of $a$ is } f\}$.
\end{definition}

\noindent
We define an operator $\sigma: 2^{\mathcal{H}} \mapsto \mathcal{H}$ which maps a conjunction to a program such that (i) for any conjunction $c$ with head predicate symbol $f$, $M(c, f)=M(\sigma(c), f)$,
% \ac{h is overused as it often means hypothesis, I suggest using a different symbol}
% \ac{@CH this statement does not hold as we need to rename the predicate symbols in a conjunction. We do not need to say this statement.}.
and (ii) for any conjunctions $c_1$ and $c_2$ such that $size(c_1) < size(c_2)$, $size(\sigma(c_1)) < size(\sigma(c_2))$.
In the following, when we say that a conjunction  \emph{$c$ is in a program $h$}, or $c \subseteq h$, we mean \emph{$\sigma(c) \subseteq h$}.

For instance, let $\sigma$ be the operator which, given a conjunction $c$ with head predicate symbol $f$ of arity $a$, returns the program obtained by (i) for each program $p \in c$, replacing each occurrence of $f$ in $p$ by a new predicate symbol $f_i$, and (ii) adding the rule $f(x_1, \dots, x_a) \leftarrow f_1(x_1, \dots, x_a), \dots, f_n(x_1, \dots, x_a)$ where $x_i, \dots, x_a$ are variables.
\begin{example}
Consider the following conjunction:
\[\begin{array}{l}
c_1 = \left\{
    \begin{array}{l}
     \left\{
    \begin{array}{l}
\emph{zendo(S) $\leftarrow$ piece(S,B), blue(B)}\\
    \end{array}
    \right\}\\
    \left\{
    \begin{array}{l}
\emph{zendo(S) $\leftarrow$ piece(S,R), red(R)}\\
    \end{array}
    \right\}
    \end{array}
    \right\}
    \end{array}
\]
Then $\sigma(c_1)$ is:
\[
\begin{array}{l}
\left\{
    \begin{array}{l}
\emph{zendo(S) $\leftarrow$ zendo$_1$(S),zendo$_2$(S)}\\
\emph{zendo$_1$(S) $\leftarrow$ piece(S,B), blue(B)}\\
\emph{zendo$_2$(S) $\leftarrow$ piece(S,R), red(R)}\\
\end{array}
\right\}
\end{array}
\]

\noindent
Consider the following conjunction:
\[\begin{array}{l}
c_2 = \left\{
    \begin{array}{l}
     \left\{
    \begin{array}{l}
\emph{f(S) $\leftarrow$ head(S,1)}\\
\emph{f(S) $\leftarrow$ tail(S,T),f(T)}\\
    \end{array}
    \right\}\\
    \left\{
    \begin{array}{l}
\emph{f(S) $\leftarrow$ head(S,2)}\\
\emph{f(S) $\leftarrow$ tail(S,T),f(T)}\\
    \end{array}
    \right\}
    \end{array}
    \right\}
    \end{array}
\]
Then $\sigma(c_2)$ is:
\[
\begin{array}{l}
\left\{
    \begin{array}{l}
\emph{f(S) $\leftarrow$ f$_1$(S),f$_2$(S)}\\
\emph{f$_1$(S) $\leftarrow$ head(S,1)}\\
\emph{f$_1$(S) $\leftarrow$ tail(S,T),f$_1$(T)}\\
\emph{f$_2$(S) $\leftarrow$ head(S,2)}\\
\emph{f$_2$(S) $\leftarrow$ tail(S,T),f$_2$(T)}\\
\end{array}
\right\}
\end{array}
\]
% \ac{I would use the zendo example from section 1 of the paper}
\end{example}
% \ac{|@CH, add a recursive example}

\noindent
The generate stage of \combo{} generates non-separable programs.
We recall the definition of a separable program:
\begin{definition}
[\textbf{Separable program}]
A program $h$ is \emph{separable} when (i) it has at least two rules, and (ii) no predicate symbol in the head of a rule in $h$ also appears in the body of a rule in $h$. A program is \emph{non-separable} when it is not separable.
\end{definition}

\subsection{Generate and Test}
\noindent
We show that \name{} can generate and test every non-splittable non-separable program:
\begin{proposition}[\textbf{Correctness of the generate and test stages}]
\label{lem_generate}
\name{} can generate and test every non-splittable non-separable program.
\end{proposition}
\begin{proof}
Cropper and Hocquette \shortcite{combo} show (Lemma 1) that \combo{} can generate and test every non-separable program under Assumption \ref{decidable}.
% the generate encoding of \combo{} has a model for every program in the hypothesis space.
The constraint we add to the generate encoding (Section \ref{generate}) prunes splittable programs.
% a subset of all non-separable programs.
Therefore \name{} can generate and test every non-splittable non-separable program.
\end{proof}

\subsection{Join}
Proposition \ref{lem_generate} shows that \name{} can generate and test every non-splittable non-separable program. 
However, the generate stage cannot generate splittable non-separable programs.
To learn a splittable non-separable program, \name{} uses the join stage to join non-splittable programs into splittable programs.
To show the correctness of this join stage, we first show that the logical consequences of a rule which body is the conjunction of the body of two rules $r_1$ and $r_2$ is equal to the intersection of the logical consequences of $r_1$ and $r_2$: 
% \ac{can you add more text here to help a reader beforehand? what is the high-level idea?}
% We introduce a Lemma to show this result:

% \begin{lemma}
% % [\textbf{Conjunction of non-splittable rules}]
% \label{eq}
% Let 
% $r_1 = (g \leftarrow L_1)$, 
% $r_2 = (g \leftarrow L_2)$, 
% and $r = (g \leftarrow L_1, L_2)$ be three rules, such that the body-only variables of $r_1$ and $r_2$ are distinct.
% Then $M_{\{g\}}(r) = M_{\{g\}}(\sigma(r_1 \cup r_2))$.
% \end{lemma}
% \begin{proof}
% Follows from the correctness of the unfold operator.
% \end{proof}

% Let $a \in M(r_1) \cap M(r_2)$. We show $a \in M(r)$. 


% \begin{lemma}
% Let 
% $r_1 = (g \leftarrow L_1)$, 
% $r_2 = (g \leftarrow L_2)$, 
% and $r = (g \leftarrow L_1, L_2)$ be three rules, such that the body-only variables of $r_1$ and $r_2$ are distinct.
% Then $M(r) = M(r_1) \cap M(r_2)$.
% \end{lemma}
% \begin{proof}
% \begin{align*}
% \end{align*}
% Let $M_{r_1 \cap r_2} = M(r_1) \cap M(r_2)$.
% We know that $M(r_1)$ is equal to the consequences of $r$ without the consequences of $r_2$, without the consequences of $r_1 \cap r_2$:
% \begin{align*}
% M(r_1) = (M(r)\setminus M(r_2))\cup (M(r_1)\cap M(r_2))
% \end{align*}
% Similarly for $M(r_2)$:
% \begin{align*}
% M(r_2) = (M(r)\setminus M(r_1))\cup (M(r_2)\cap M(r_1))
% \end{align*}
% Then:
% \begin{align}
% M(r) =& (M(r)\setminus M(r_2))\cup (M_{r_1 \cap r_2}) \\
% &\cap (M(r)\setminus M(r_1))\cup (M_{r_1 \cap r_2}) \\
% &=  (M(r) \setminus M(r_2)  \cap  M(r) \setminus M(r_1) )  \cup  (M_{r_1 \cap r_2})
% \end{align}

% We know $M(r)\setminus M(r_2)  \cap  M(r)\setminus M(r_1)  = \emptyset$. Then:
% \begin{align*}
% M(r) = (M_{r_1 \cap r_2})
% \end{align*}
% % \begin{align}
% % M(r) =& (M(r)\setminus M(r_1) \cup M(r) \setminus M(r_2)) \cup M_{r_1 \cap r_2}\\
% % =& (M(r)\setminus (M(r_1) \setminus M_{r_1 \cap r_2}) \cup M_{r_1 \cap r_2})\\
% % &\cap (M(r) \setminus (M(r_2)\setminus M_{r_1 \cap r_2}) \cup M_{r_1 \cap r_2} )\\
% % =& (M(r_1) \cup M_{r_1 \cap r_2}) \cap (M(r_2) \cup M_{r_1 \cap r_2})\\
% % =& M(r_1) \cap M(r_2)
% % \end{align}

% \end{proof}
% \begin{align*}
% M(r) = (M(r)/M(c1) \cap M(r)/M(c2)) \cup (M(c1) \cap M(c2)
% \end{align*}
% \begin{align*}
% % M(c) = M(c1) \cap M(c2).\\
% M(r) = (M(r)/(M(c1)/(M(c1) \cap M(c2)))\\ \cap M(r)/(M(c2)/(M(c1) \cap M(c2)))\\
% \cup (M(c1) \cap M(c2)).\\
% Concerning M(r)/(M(c1)/(M(c1) \cap M(c2)))\\ M(r)/(M(c2)/(M(c1) \cap M(c2))),\\
% \text{these sets are mutually exclusive}\\ \text{and thus have empty intersection.}\\
% \text{Furthermore,} M(r) = M(r)/(M(c1)/(M(c1) \cap M(c2)))\\
% \cap M(r)/(M(c2)/(M(c1) \cap M(c2)))\\
% \cup (M(c1) \cap M(c2)) = (M(r)/(M(c1)/(M(c1) \cap M(c2)))\\
% \cup (M(c1) \cap M(c2)) ) \cap (M(r)/(M(c2)/(M(c1) \cap M(c2))\\
% \cup (M(c1) \cap M(c2)) )\\
% = M(c1) \cap M(c2).
% \end{align*}


% \begin{lemma}
% Let 
% $r_1 = (g \leftarrow L_1)$, 
% $r_2 = (g \leftarrow L_2)$, 
% and $r = (g \leftarrow L_1, L_2)$ be three rules, such that the body-only variables of $r_1$ and $r_2$ are distinct.
% Let $c$ be the conjunction of $r_1$ and $r_2$.
% Then $M(r) = M(c)$.
% \end{lemma}
% \begin{proof}
% Follows from the correctness of the unfold operator.
% \end{proof}


\begin{lemma}
% [\textbf{Conjunction of non-splittable rules}]
\label{eq}
Let 
$r_1 = (g \leftarrow L_1)$, 
$r_2 = (g \leftarrow L_2)$, 
and $r = (g \leftarrow L_1, L_2)$ be three rules, such that the body-only variables of $r_1$ and $r_2$ are distinct.
% and $c_1, c_2,$ and $c$ be three conjunctions such that 
% $c = c_1 \cup c_2$,
% $M(r_1) = M(c_1)$, 
% $M(r_2) = M(c_2)$,
Then $M(r) = M(r_1) \cap M(r_2)$.
\end{lemma}
% \begin{proof}
% \begin{align*}
% M(c) &= \cap_{p \in c} M(p)\\
% &= (\cap_{p \in c_1} M(p)) \cap (\cap_{p \in c_2} M(p))\\
% &= M(c_1) \cap M(c_2)\\
% &= M(r_1) \cap M(r_2)\\
% \end{align*}
% Then $\sigma(c)$ is:
% \[
% \begin{array}{l}
% \left\{
%     \begin{array}{l}
% \emph{$g \leftarrow g_{1,1},\dots, g_{1,l}, g_{2,1},\dots, g_{2,m}$}\\
% \end{array}
% \right\}
% \end{array}
% \]
% where $g_{1,i} \leftarrow M_i$ with $M_i \subseteq L_1$ and $\cup_{i} M_i = L_1$\\
% and $g_{2,i} \leftarrow M_j$ with $M_j \subseteq L_2$ and $\cup_{j} M_2= L_2$\\
% From the correctness of the unfold operator, we have:
% Then $\sigma(c)$ is equivalent to:
% \[
% \begin{array}{l}
% \left\{
%     \begin{array}{l}
% \emph{$g \leftarrow L_1, L_2$}\\
% \end{array}
% \right\}
% \end{array}
% \]
% \end{proof}

\begin{proof}
% a in mc implies a in mr
We first show that if $a\in~M(r)$ then $a~\in M(r_1)~\cap~M(r_2)$.
The rule $r$ specialises $r_1$ which implies that $M(r)\subseteq~M(r_1)$ and therefore $a \in M(r_1)$.
Likewise, $r$ specialises $r_2$ which implies that $M(r) \subseteq M(r_2)$ and therefore $a \in M(r_2)$. 
Therefore $a \in M(r_1) \cap M(r_2)$.
% Since the body-only variables of $r_1$ and $r_2$ are distinct the logical consequences are independent.
% \ac{@AC, confused myself}

We now show that if $a \in M(r_1) \cap M(r_2)$ then $a \in M(r)$. 
Since $a \in M(r_1)$ then $L_1 \lor \neg g \models a$. 
Similarly, since $a \in M(r_2)$ then $L_2 \lor \neg g \models a$. 
Then $(L_1 \lor \neg g) \land (L_2 \lor \neg g) \models a$ by monotonicity, and $a \in M(r)$. 
% \ch{still very unsure about how to prove that}
% \ac{it also does not seem correct as a is defined with the predicate symbol of g}
\end{proof}
% OLD
% \begin{proof}
% % a in mc implies a in mr
% We first show that if $a \in M(c)$ then $a \in M(r)$.
% Let $a \in M(c)$. 
% % \ac{Since c is the intersection of ?}
% Since, $c_1 \subseteq c$ then, by Definition \ref{conjunction}, $a \in M(c_1)$ which implies that $a \in M(r_1)$.
% and $L_1 \lor \neg f \models a$. 
% Similarly, $c_2 \subseteq c$ then, by Definition \ref{conjunction}, $a \in M(c_2)$ which implies that $a \in M(r_2)$
% and $L_2 \lor \neg f \models a$. 
% Then $(L_1 \lor \neg f) \land (L_2 \lor \neg f) \models a$ since the body-only variables of $r_1$ and $r_2$ are distinct, and $a \in M(r)$. \ch{I am unsure about this last step}

% a not in mc implies a not in mr
% \ac{We show that if $a \not\in M(c)$ then $a \not\in M(r)$. }

% a in mr implies a in mc
% \ac{We show that if $a \in M(r)$ then $a \in M(c)$. }
% Let $a \in M(r)$. 
% Then $(L_1 \land L_2) \lor \neg f \models a$, therefore $(L_1 \lor \neg f) \land (L_2 \lor \neg f) \models a$.
% Then, $a \in M(r_1)$ and $a \in M(r_2)$,
% thus $a \in M(c_1)$ and $a \in M(c_2)$. 
% Then, $a \in M(c)$, and $M(r) = M(c)$.

% a not in mr implies a not in mc
% \ac{We show that if $a \not\in M(r)$ then $a \not\in M(c)$. }


% \ch{initial proof}
% Let $a \in M(c)$. Then, $a \in M(c_1)$. Then, $a \in M(r_1)$.
% Then $L_1 \lor \neg f \models a$. Similarly, $a \in M(c_2)$, therefore $a \in M(r_2)$, and $L_2 \lor \neg f \models a$. Then $(L_1 \lor \neg f) \land (L_2 \lor \neg f) \models a$ since the body-only variables of $r_1$ and $r_2$ are distinct, and $a \in M(r)$. \ch{I am unsure about this last step}
% % Let $a \in M(c)$. Then, $a \in M(c_1)$ and $a \in M(c_2)$. Then, $a \in M(r_1)$ and $a \in M(r_2)$.
% % Then $L_1 \lor \neg h \models a$.

% Let $a \in M(r)$. 
% Then $(L_1 \land L_2) \lor \neg f \models a$, therefore $(L_1 \lor \neg f) \land (L_2 \lor \neg f) \models a$.
% Then, $a \in M(r_1)$ and $a \in M(r_2)$,
% thus $a \in M(c_1)$ and $a \in M(c_2)$. 
% Then, $a \in M(c)$, and $M(r) = M(c)$.
% \end{proof}

\noindent
With this result, we show that any rule is equivalent to a conjunction of non-splittable programs:
\begin{lemma}[\textbf{Conjunction of non-splittable programs}]
\label{lem_splittable}
% Let $r=(h,b)$ be a rule with head $h = f(A,B,...)$ of arity $a$ and with body $b$. Then $r$ can be decomposed as $h\leftarrow inv_1(A,B,...), inv_2(A,B,...), ...$ where each $inv_i$ is a new predicate symbol not appearing in $r$ and with arity $a$ and each $inv_i(A,B,...)$ is defined with a non-splittable rule with literals from $b$ in its body.
% Then $b = \bigcup_{i=1}^n b_{i}$ where each rule with head $h$ and body $b_{i}$ is a non-splittable rule.
Let $r$ be a rule. Then there exists a conjunction $c$ of non-splittable programs such that $M(r) = M(c)$.
\label{rules}
\end{lemma}

% \begin{proof}
% \ch{NEEEW}
% We prove the result by induction on the number of body literals $m$ in the body of $r$. 

% For the base case, if $m=1$ then $r$ is non-splittable. 
% Let $c$ be the conjunction $\{\{r\}\}$. 
% Then $M(r) = M(c)$.
% % \ac{M(c) is really confusing as c is a set of sets. I know we redefine M(c) for a conjunction but it is confusing. I am unsure what to do.}

% For the inductive case, assume the claim holds for rules with $m$ body literals.
% % We show the claim holds for rules with $m+1$ body literals.
% Let $r$ be a rule with $m+1$ body literals.
% Either $r$ is (i) non-splittable, or (ii) splittable.
% For case (i), assume $r$ is non-splittable. Let $c$ be the conjunction $\{\{r\}\}$. Then $M(r) = M(c)$.
% For case (ii), assume $r$ is splittable. 
% Then, by Definition \ref{def:splittablerule}, its body literals can be partitioned into two non-empty sets $L_1$ and $L_2$ such that the body-only variables in $L_1$ are disjoint from the body-only variables in $L_2$.
% Both $L_1$ and $L_2$ have fewer than $m$ literals.
% Let $a$ be the head literal of $r$.
% Let $r_1 = (a_1 \leftarrow L_1)$, $r_2 = (a_2 \leftarrow L_2)$, $r_3 = (a \leftarrow a_1, a_2)$. 
% By the induction hypothesis, there exists a conjunction $c_1$ of non-splittable programs such that $M(r_1)=M(c_1)$ and a conjunction $c_2$ of non-splittable programs such that $M(r_2)=M(c_2)$.
% Let $c = r_1 \cup r_2 \cup r_3$.
% $M(r)=M_{\{a\}}(c)$ from the correctness of the unfold operator.
% but these rules are not splittable and c is not a conjunction
% \end{proof}

\begin{proof}
We prove the result by induction on the number of body literals $m$ in the body of $r$. 

For the base case, if $m=1$ then $r$ is non-splittable. 
Let $c$ be the conjunction $\{\{r\}\}$. 
Then $M(r) = M(c)$.
% \ac{M(c) is really confusing as c is a set of sets. I know we redefine M(c) for a conjunction but it is confusing. I am unsure what to do.}

For the inductive case, assume the claim holds for rules with $m$ body literals.
% We show the claim holds for rules with $m+1$ body literals.
Let $r$ be a rule with $m+1$ body literals.
Either $r$ is (i) non-splittable, or (ii) splittable.
For case (i), assume $r$ is non-splittable. Let $c$ be the conjunction $\{\{r\}\}$. Then $M(r) = M(c)$.
For case (ii), assume $r$ is splittable. 
Then, by Definition \ref{def:splittablerule}, its body literals can be partitioned into two non-empty sets $L_1$ and $L_2$ such that the body-only variables in $L_1$ are disjoint from the body-only variables in $L_2$.
Both $L_1$ and $L_2$ have fewer than $m$ literals.
Let $a$ be the head literal of $r$.
Let $r_1 = (a \leftarrow L_1)$ and $r_2 = (a \leftarrow L_2)$. 
By the induction hypothesis, there exists a conjunction $c_1$ of non-splittable programs such that $M(r_1)=M(c_1)$ and a conjunction $c_2$ of non-splittable programs such that $M(r_2)=M(c_2)$.
Let $c = c_1 \cup c_2$. 
Then $c$ is a conjunction because the programs in $c_1$ and $c_2$ have the same head predicate symbol.
From Lemma \ref{eq}, $M(r)=M(r_1) \cap M(r_2)$ and therefore $M(r)=M(c_1) \cap M(c_2)=M(c)$ which completes the proof.
\end{proof}

\begin{myexample}[\textbf{Conjunction of non-splittable programs}] \label{ex1}
Consider the rule $r$:
\[
    \begin{array}{l}
    r = \left\{
    \begin{array}{l}
\emph{f(A) $\leftarrow$ head(A,1),tail(A,B),head(B,3)}\\
    \end{array}
    \right\}\\
    \end{array}
\]
Consider the non-splittable programs:
\[
    \begin{array}{l}
    p_1 = \left\{
    \begin{array}{l}
\emph{f(A) $\leftarrow$ head(A,1)}\\
    \end{array}
    \right\}\\
    p_2 = \left\{
    \begin{array}{l}
\emph{f(A) $\leftarrow$ tail(A,B),head(B,3)}\\
    \end{array}
    \right\}
    \end{array}
\]
Then $M(r) = M(c)$ where $c$ is the conjunction $c=p_1 \cup p_2$.
\end{myexample}

\noindent
We show that any program is equivalent to a conjunction of non-splittable programs:
\begin{lemma}[\textbf{Conjunction of non-splittable programs}]
\label{lem_splittable_program}
Let $h$ be a program. Then there exists a conjunction $c$ of non-splittable programs such that $M(h) = M(c)$.
\end{lemma}
\begin{proof}
$h$ has either (i) at least two rules, or (ii) one rule.
For case (i), if $h$ has at least two rules, then $h$ is non-splittable. Let $c$ be the conjunction $\{\{h\}\}$. Then $M(h) = M(c)$.
For case (ii), Lemma \ref{rules} shows there exists a conjunction $c$ of non-splittable programs such that $M(h) = M(c)$.
\end{proof}
% \ch{do we also need something about the size of the conjunction?}

\noindent
The join stage takes as input \emph{joinable} programs. We define a \emph{joinable} program:
\begin{definition}[\textbf{Joinable program}]
 A program is \emph{joinable} when it (i) is non-splittable, (ii) is non-separable, (iii) entails at least one positive example, and (iv) entails at least one negative example.
 % ($tp > 0$).
\end{definition}

\noindent
The combine stage takes as input \emph{combinable} programs. We define a \emph{combinable} program:
\begin{definition}[\textbf{Combinable program}]
A program is \emph{combinable} when it (i) is non-separable, (ii) entails at least one positive example, and (iii) entails no negative example.
\end{definition}

\noindent
We show that any combinable program is equivalent to a conjunction of non-splittable non-separable programs which each entail at least one positive example:
\begin{lemma}[\textbf{Conjunction of programs}]\label{lem_opti_separable}
Let $h$ be combinable program. Then there exists a conjunction $c$ of programs such that $M(c)=M(h)$ and each program in $c$ (i) is non-splittable, (ii) is non-separable, and (iii) entails at least one positive example.
\end{lemma}

\begin{proof}
From Lemma \ref{lem_splittable_program}, there exists a conjunction $c$ of non-splittable programs such that $M(c)=M(h)$.
For contradiction, assume some program $h_i \in c$ is either (i) separable, or (ii) does not entail any positive example. 
For case (i), assume that $h_i$ is separable. 
Then $h_i$ has at least two rules and therefore cannot be non-splittable, which contradicts our assumption.
For case (ii), assume $h_i$ does not entail any positive example.
Then $c$ does not entail any positive example and $h$ does not entail any positive example. 
Then $h$ is not a combinable program, which contradicts our assumption.
Therefore, each $h_i \in c$ (i) is non-splittable, (ii) is non-separable, and (iii) entails at least one positive example.
\end{proof}

\noindent
The join stage returns non-subsumed conjunctions. A conjunction is subsumed if it entails a subset of the positive examples entailed by a strictly smaller conjunction:
% entails a subset of the positive examples entailed by a strictly smaller conjunction 
\begin{definition}[\textbf{Subsumed conjunction}] Let $c_1$ and $c_2$ be two conjunctions which do not entail any negative examples,
$c_1 \models E^{+}_1$,
$c_2 \models E^{+}_2$,
$E^{+}_2 \subseteq E^{+}_1$,
$size(c_1) < size(c_2)$. Then $c_2$ is subsumed by $c_1$.
\end{definition}

% \ch{does the following result help to prove the next proposition (correctness of the join stage)? the join stage only takes as input programs which cover at least one neg ex and returns conjunctions of at least two programs}
% \ch{should 'joinable' (def 6) also cover some negative examples?}
\begin{lemma}[\textbf{Conjunction of joinable programs}]\label{lem_splittable_separable}
Let $h$ be a non-subsumed splittable combinable program. Then there exists a conjunction $c$ of joinable programs such that $M(c)=M(h)$.
\end{lemma}
\begin{proof}
Since $h$ is splittable, $h$ has a single rule which body literals can be partitioned into two non-empty sets $L_1$ and $L_2$ such that the body-only variables in $L_1$ are disjoint from the body-only variables in $L_2$. Let $g$ be the head literal of the rule in $h$. Let $r_1 = (g \leftarrow L_1)$ and $r_2 = (g \leftarrow L_2)$. 
From Lemma \ref{lem_opti_separable}, there exists two conjunctions $c_1$ and $c_2$ such that $M(c_1)=M(r_1)$ and $M(c_2)=M(r_2)$ and each program in $c_1 \cup c_2$ (i) is non-splittable, (ii) is non-separable, and (iii) entails at least one positive example.
Let $c = c_1 \cup c_2$. Then $c$ is a conjunction because the programs in $c_1$ and $c_2$ have the same head predicate symbol. 
From Lemma \ref{eq}, $M(r)=M(r_1) \cap M(r_2)$ and therefore $M(r) = M(c_1) \cap M(c_2) = M(c)$.
Therefore there exists a conjunction $c$ of at least two programs such that $M(c)=M(h)$ and each program in $c$ (i) is non-splittable, (ii) is non-separable, and (iii) entails at least one positive example.
Assume some $h_i \in c$ does not cover any negative example.
Then the conjunction $c' = \{\{h_i\}\}$ does not entail any negative example. Since $c$ has at least two elements, then $c' \subset c$, and $c$ is subsumed by $c'$ which contradicts our assumption. Therefore, each $h_i \in c$ entails some negative examples and is joinable.
\end{proof}

\noindent
We show that the join stage returns all non-subsumed splittable combinable programs:
\begin{proposition}[\textbf{Correctness of the join stage}]
\label{lem_join}
% Let $h$ be a splittable combinable program. Given the set of all joinable programs, the join stage returns a conjunction $c$ such that $M(c) = M(h)$.\ac{OLD}
Given all joinable programs, the join stage returns all non-subsumed splittable combinable programs.
% \ac{NEW}
% s all splittable combinable programs.
\end{proposition}
\begin{proof}
Assume the opposite, i.e. that there is a non-subsumed splittable combinable program $h$ not returned by the join stage.
As $h$ is non-subsumed splittable combinable, by Lemma \ref{lem_splittable_separable}, there exists a conjunction $c$ of joinable programs such that $M(c)=M(h)$. 
As $h$ is non-subsumed, $c$ is not subsumed by another conjunction.
The join stage uses a SAT solver to enumerate maximal satisfiable subsets \cite{DBLP:journals/jar/LiffitonS08} corresponding to the subset-maximal coverage of conjunctions.
As we have all joinable programs, the solver will find every conjunction of joinable programs not subsumed by another conjunction.
Therefore, the solver finds $c$ and the join stage returns $h$, which contradicts our assumption.



% which implies the join stage does not return a conjunction $c$ such that $M(c) = M(h)$.
% For contradiction, assume the opposite, which implies the join stage does not return a conjunction $c$ such that $M(c) = M(h)$.
% there exists a splittable combinable program $h$ such that the join stage does not return a program equivalent to $h$.

% For all $h_i \in c$, then $h_i$.
% Since $h$ is combinable, $h$ entails at least one positive example. 
% There are finitely many joinable programs. 
% Moreover, since $h$ is combinable, $c$ is a model for the SAT encoding.
% The SAT solver finds all models that entails at least one positive example and no negative examples.
% Therefore the SAT solver finds $c$.
% The assumption cannot hold and the join stage returns a conjunction $c$ such that $M(c) = M(h)$.
% \ch{slightly unclear, needs rephrasing, as we find c not h}
% \ac{ASP to SAT?}
\end{proof}


\subsection{Combine}

% Let $\sigma$ be an operator which maps subsets of $\mathcal{H}$ to programs, i.e. sets of programs to programs such that $M(P) = M(\sigma(P))$.

% We define an operator $\sigma: 2^{\mathcal{H}} \mapsto \mathcal{H}$ which maps subsets of $\mathcal{H}$ to programs \ac{NEW???}

% In the following, we say \emph{c is in a program} to mean \emph{$\sigma(c) \in P$}.

% \ch{need to show such an operator exists}
% \ac{we need to define it}
% \ch{say something about the size of conjunctions?}
% \ac{operator should probably go in with the definition of a conjunction}

\noindent
We first show that a subsumed conjunction cannot be in an optimal solution:
\begin{proposition}[\textbf{Subsumed conjunction}]
\label{prop_subsumed}
Let $c_1$ and $c_2$ be two conjunctions such that $c_2$ is subsumed by $c_1$,
% which do not entail any negative examples,
% $c_1 \models E^{+}_1$,
% $c_2 \models E^{+}_2$,
% $E^{+}_2 \subseteq E^{+}_1$,
% $size(c_1) < size(c_2)$,
$h$ be a solution, 
and $\sigma(c_2) \subseteq h$.
Then $h$ cannot be optimal.
\end{proposition}
\begin{proof}
% Assume there exists an optimal solution $h_o$ and a hypothesis $h$ such that $h_o = c_2 \cup h$.
Assume the opposite, i.e. $h$ is an optimal solution.
% Assume there exists an optimal solution $h_o$ and a hypothesis $h$ such that $h_o = h \cup \sigma{}(c_2)$.
% We show that $h'_o = c_1 \cup h$ is a solution.
We show that $h' = (h \setminus \sigma(c_2)) \cup \sigma(c_1)$ is a solution.
Since $h$ is a solution, it does not entail any negative examples.
Therefore, $h \setminus \sigma(c_2)$ does not entail any negative examples. 
Since $c_1$ does not entail any negative examples, then $h'$ does not entail any negative examples.
Since $h$ is a solution, it entails all positive examples. 
Since $E^{+}_2 \subseteq E^{+}_1$, $h'$ also entails all positive examples.
Therefore $h'$ is a solution.
Since $size(c_1) < size(c_2)$ then $size(h') < size(h)$. 
Then $h$ cannot be optimal, which contradicts our assumption.
\end{proof}

\begin{corollary}
Let $c_1$ and $c_2$ be two conjunctions which do not entail any negative examples,
% and entail the positive examples $E^{+}_1$ and $E^{+}_2$ respectively, and
% which entail the positive examples 
$c_1 \models E^{+}_1$,
$c_2 \models E^{+}_2$,
% and $E^{+}_2$ respectively and no negative example, 
% such that
$E^{+}_2 \subseteq E^{+}_1$, 
and $size(c_1) < size(c_2)$. 
Then $c_2$ cannot be in an optimal solution.
\label{coro:subsumed}
\end{corollary}

\begin{proof}
Follows from Proposition \ref{prop_subsumed}.
\end{proof}


% \noindent
% We show the correctness of the combine stage. 
\noindent
With this result, we show the correctness of the combine stage:
\begin{proposition}[\textbf{Correctness of the combine stage}] \label{prop_combine}
Given all non-subsumed combinable programs, the combine stage returns an optimal solution.
\end{proposition}
\begin{proof}
Cropper and Hocquette [\citeyear{combo}] show that given all combinable programs, the combine stage returns an optimal solution under Assumption \ref{independentbk}. Corollary \ref{coro:subsumed} shows that subsumed conjunctions cannot be in an optimal solution. 
Therefore, the combine stage of \name{} returns an optimal solution given all non-subsumed combinable programs.
\end{proof}

% \noindent
% We show that \name{} (with only the generate, test, join and combine stages) returns a solution:
% \begin{lemma}[\textbf{Correctness of \name{} without constraints}]
% \label{lem_gen_one_opt}
% \name{} returns a solution.
% \end{lemma}
% \begin{proof}
% For contradiction, assume the opposite, i.e. \name{} does not return a solution.
% This assumption implies that \name{} (i) returns a hypothesis that is not a solution, or (ii) does not return a hypothesis.
% Case (i) cannot hold because as an output of the combine stage $h$ is complete and consistent so is a solution. 
% Case (ii) cannot hold because 
% Lemma \ref{lem_generate} shows that \name{} can generate and test every non-splittable non-separable program, of which there are finitely many.
% Lemma \ref{lem_join} shows that the join stage can build every splittable combinable program, of which there are finitely many.
% Therefore, \name{} can generate every combinable program.
% Given the set of all combinable programs, the combine stage returns a solution \cite{combo}.
% By Assumption \ref{existencesol}, a solution exists.
% Therefore \name{} returns a solution.
% \end{proof}

% \noindent
% We show that \name{} without constraints returns an optimal solution.
% \begin{proposition}[\textbf{Correctness of \name{} without constraints}]
% \label{prop1}
% \name{} without constraints returns an optimal solution.
% \end{proposition}
% \begin{proof}
% Follows from Lemma \ref{lem_gen_one_opt} and that \name{} uses iterative deepening over the program size to guarantee optimality.
% \end{proof}


\subsection{Constrain}

% In the previous section, we showed that \name{} finds an optimal solution when it does not apply any constraints.
In this section, we show that the constrain stage never prunes optimal solutions from the hypothesis space.
\name{} builds specialisations constraints from non-splittable non-separable programs that do not entail (a) any positive example, or (b) any negative example. 
% Moreover, \name{} does not build subsumed conjunctions (constraint (c)).

% \noindent
We show a result for case (a). If a hypothesis does not entail any positive example, \name{} prunes all its specialisations, as they cannot be in a conjunction in an optimal solution:
\begin{proposition}[\textbf{Specialisation constraint when tp=0}]
\label{prop:totincomplete}
% Let $h_1$ be a hypothesis that does not entail any positive example 
% and $h_2$ be a specialisation of $h_1$.
% Then $h_2$ cannot be in a conjunction $c$ such that $\sigma(c)$ is in an optimal solution.
% \ac{NEW}
% Let $h_1$ be a hypothesis that does not entail any positive example,
% $h_2$ be a specialisation of $h_1$, 
% $h_o$ be an optimal solution, 
% $c$ be a conjunction,
% and $\sigma(c) \subseteq{} h_o$.
% Then $h_2 \not\in c$.
% NEW2
% Let $h_1$ be a hypothesis that does not entail any positive example,
% $h_2$ be a specialisation of $h_1$, 
% $h$ be a hypothesis,
% $c$ be a conjunction,
% and $\sigma(c) \subseteq{} h_o$.
% Then $h_2 \not\in c$.
% NEW3 
Let $h_1$ be a hypothesis that does not entail any positive example,
$h_2$ be a specialisation of $h_1$, 
$c$ be a conjunction,
$h_2 \in c$,
$h$ be a solution,
and $\sigma{}(c) \subseteq{} h$.
Then $h$ is not an optimal solution.
\end{proposition}
\begin{proof}
% OLD
% Assume the opposite, i.e. there exists an optimal solution $h_o$ and a conjunction $c$ such that $h_2 \in c$ and $\sigma{}(c) \subseteq h_o$. 
% NEW
% Assume the opposite, i.e. $h_2 \in c$.
Assume the opposite, i.e. $h$ is an optimal solution.
We show that $h' = h \setminus \sigma{}(c)$ is a solution.
% \ac{<--- @CH, when the assumptions are in the proposition, this sentence does not make sense}
Since $h$ is a solution, it does not entail any negative example. Then $h'$ does not entail any negative example.
Since $h_1$ does not entail any positive example and $h_2$ specialises $h_1$ then $h_2$ does not entail any positive example. Then $c$ does not entail any positive example. 
Since $h$ entails all positive examples and $c$ does not entail any positive example, then $h'$ entails all positive examples.
Since $h'$ entails all positive examples and no negative examples, it is a solution.
Moreover, $size(h') < size(h)$.
Then $h$ cannot be optimal, which contradicts our assumption.
\end{proof}

\begin{corollary}
% [\textbf{Specialisation constraint when tp=0}]
Let $h_1$ be a hypothesis that does not entail any positive example
and $h_2$ be a specialisation of $h_1$.
Then $h_2$ cannot be in a conjunction in an optimal solution.
\label{cor_totincomplete}
\end{corollary}
\begin{proof}
Follows from Proposition \ref{prop:totincomplete}.
\end{proof}

% \begin{myexample}[\textbf{Specialisation constraint when tp=0}]
% % [
% % \textbf{Specialisations of totally incomplete programs}]
%     Consider the hypothesis:
% \[
%     \begin{array}{l}
%     h_1 = \left\{
%     \begin{array}{l}
%     \emph{f(A,B) $\leftarrow$ head(A,B)}
%     \end{array}
%     \right\}
%     \end{array}
% \]
% If $h_1$ does not entail any positive example, we can prune its specialisations, such as the $h_2$, as they cannot be in a conjunction of an optimal solution.
% \[
%     \begin{array}{l}
%     h_2 = \left\{
%     \begin{array}{l}
%     \emph{f(A,B) $\leftarrow$ head(A,B), even(B)}
%     \end{array}
%     \right\}
%     \end{array}
% \]
% For instance, $h_3$ cannot be an optimal solution:
% \[
%     \begin{array}{l}
%     h_3 = \left\{
%     \begin{array}{l}
%     \emph{f(A,B) $\leftarrow$ f1(A,B),f2(A,B)}\\
%     \emph{f1(A,B) $\leftarrow$ head(A,B), even(B)}\\
%     \emph{f2(A,B) $\leftarrow$ last(A,C), odd(C)}\\
%     \emph{f(A,B) $\leftarrow$ tail(A,C), head(C,B)}
%     \end{array}
%     \right\}
%     \end{array}
% \]
% \noindent
% It is important to note that case (a) does not prohibit specialisations of $h_1$ from being in a non-splittable rule of an optimal solution, such as:
% \[
%     \begin{array}{l}
%     h_3 = \left\{
%     \begin{array}{l}
%     \emph{f(A,B) $\leftarrow$ head(A,B), odd(B)}\\
%     \emph{f(A,B) $\leftarrow$ tail(A,C), f(C,B)}\\
%     \end{array}
%     \right\}
%     \end{array}
% \]
% \end{myexample}

\noindent
We show a result for case (b). If a hypothesis does not entail any negative example, \name{} prunes all its specialisations, as they cannot be in a conjunction in an optimal solution:
\begin{proposition}[\textbf{Specialisation constraint when fp=0}]
\label{prop:consistent}
% OLD
% Let $h_1$ be a hypothesis that does not entail any negative example and $h_2$ be a specialisation of $h_1$.
% Then $h_2$ cannot be in a conjunction $c$ such that $\sigma(c)$ is in an optimal solution.
% Let $h_1$ be a hypothesis that does not entail any negative example, 
% and $h_2$ be a specialisation of $h_1$,
% Then $h_2$ cannot be in a conjunction $c$ such that $\sigma(c)$ is in an optimal solution.
Let $h_1$ be a hypothesis that does not entail any negative example,
$h_2$ be a specialisation of $h_1$, 
$c$ be a conjunction,
$h_2 \in c$,
$h$ be a solution,
and $\sigma(c) \subseteq{} h$.
Then $h$ is not an optimal solution.
\end{proposition}
\begin{proof}
% \ac{OLD Assume the opposite, i.e. there exists an optimal solution $h_o$, a conjunction $c$, and a hypothesis $h_3$ such that $h_2 \in c$ and $h_o = h_3 \cup \sigma{}(c)$.}
% \ac{NEW: Assume the opposite, i.e. $h$ is an optimal solution.}
Assume the opposite, i.e. $h$ is an optimal solution.
Let $c'=(c \setminus \{h_2\}) \cup \{h_1\}$ and $h'=(h \setminus \sigma{}(c)) \cup \sigma{}(c')$.
We show that $h'$ is a solution.
Since $h_1$ does not entail any negative example, then $c'$ does not entail any negative example.
Since $h$ is a solution, it does not entail any negative examples.
Then $h'$ do not entail any negative example.
Since $h_2$ specialises $h_1$, then $h_1$ entails more positive examples than $h_2$. Then $c'$ entails more positive examples than $c$, and $h'$ entails more positive examples than $h$.
Since $h$ entails all positive examples then $h'$ entails all positive examples.
Since $h'$ entails all positive examples and no negative examples, it is a solution.
Since $h_2$ specialises $h_1$ then $size(h_1) < size(h_2)$ and $size(c') < size(c)$.
Therefore, $size(h') < size(h)$.
Then $h$ cannot be optimal, which contradicts our assumption.
% (i) an optimal solution or (ii) in an optimal splittable solution. For case (i), assume $h_2$ is an optimal solution. Since $h_2$ is complete and $h_2$ specialises $h_1$ then $h_1$ is complete. Since $h_1$ is complete and consistent then it is a solution. Since $h_2$ specialises $h_1$ then $size(h_1) < size(h_2)$.
% Therefore, $size(h_1) < size(h_2)$ so $h_2$ is not an optimal solution and case (i) cannot hold.
% For case (ii), assume $h_2$ is in an optimal splittable solution $h_o$.
% Then $h_o = h_2 \cup h_3$ where $h_3 \neq \emptyset$.
% Let $h' = h_1 \cup h_3$. 
% Since $h_o$ is complete and $h_2$ specialises $h_1$ then $h'$ is complete.
% Since $h_o$ is consistent then $h_3$ is consistent. Since $h_o$ is splittable and $h_2$ specialises $h_1$ then $h'$ is splittable.
% Since $h_1$ and $h_3$ are consistent and $h'$ is splittable then Lemma \ref{consistent} shows that $h'$ is consistent.
% As $h'$ is complete and consistent it is a solution.
% Since $h_2$ specialises $h_1$ then $size(h_1) < size(h_2)$.
% Therefore, $size(h') < size(h_o)$ so $h_o$ is not an optimal solution and case (ii) cannot hold.
% These cases are exhaustive so the assumption cannot hold.
\end{proof}
% \begin{example}[\textbf{Specialisation constraint when fp=0}]
% % [\textbf{Specialisations of consistent programs}] 
% Consider the hypothesis:
% \[
%     \begin{array}{l}
%     h_1 = \left\{
%     \begin{array}{l}
%     \emph{f(A,B) $\leftarrow$ head(A,B)}
%     \end{array}
%     \right\}
%     \end{array}
% \]
% If $h_1$ does not entail any negative example, we can prune its specialisations, such as $h_2$ as they cannot appear in a rule of an optimal solution:
% \[
%     \begin{array}{l}
%     h_2 = \left\{
%     \begin{array}{l}
%     \emph{f(A,B) $\leftarrow$ head(A,B), even(B)}
%     \end{array}
%     \right\}
%     \end{array}
% \]

% \noindent
% It is important to note that case (a) does not prohibit specialisations of $h_1$ from being in multi-clause non-splittable programs such as:
% \[
%     \begin{array}{l}
%     h_3 = \left\{
%     \begin{array}{l}
%     \emph{f(A,B) $\leftarrow$ head(A,B),odd(B)}\\
%     \emph{f(A,B) $\leftarrow$ tail(A,C), f(C,B)}\\
%     \end{array}
%     \right\}
%     \end{array}
% \]
% \end{example}


\noindent
If a hypothesis does not entail any negative example, \name{} prunes all its specialisations, as they cannot be in a conjunction in an optimal solution:
\begin{corollary}
% [\textbf{Specialisation constraint when fp=0}]
Let $h_1$ be a hypothesis that does not entail any negative example and $h_2$ be a specialisation of $h_1$.
Then $h_2$ cannot be in a conjunction in an optimal solution.
\label{cor_consistent}
\end{corollary}
\begin{proof}
Follows from Proposition \ref{prop:consistent}.
\end{proof}

% Constraints inferred in cases (a), (b), and (c) never prune optimal solutions from the hypothesis space.
\noindent
We now show that the constrain stage never prunes an optimal solution:

\begin{proposition}[\textbf{Optimal soundness of the constraints}]
    % [\textbf{Optimally sound constraints}]
\label{prop_opt_sound}
The constrain stage of \name{} never prunes an optimal solution.
\end{proposition}
\begin{proof}
\name{} builds constraints from non-splittable non-separable programs that do not entail (a) any positive example, or (b) any negative example.
For case (a), if a program does not entail any positive example, \name{} prunes its specialisations which by Corollary \ref{cor_totincomplete} cannot be in a conjunction in an optimal solution.
For case (b), if a program does not entail any negative example, \name{} prunes its specialisations which by Corollary \ref{cor_consistent} cannot be in a conjunction in an optimal solution.
% Moreover, \name{} does not build subsumed conjunctions, which by Proposition \ref{prop_subsumed} cannot be in an optimal solution.
Therefore, \name{} never prunes an optimal solution.
\end{proof}

\subsection{\name{} Correctness}

We show the correctness of the \name{} without the constrain stage:
\begin{proposition}[\textbf{Correctness of \name{} without the constrain stage}]
\name{} without the constrain stage returns an optimal solution.
\label{correctness}
\end{proposition}
\begin{proof}
Proposition \ref{lem_generate} shows that \name{} can generate and test all non-splittable non-separable programs.
These generated programs include all joinable programs and all non-splittable combinable programs.
% \ac{do not understand: Among which are (i) all joinable programs, and (ii) all non-splittable combinable programs.}
% Proposition \ref{lem_join} shows that given all joinable programs, for any splittable combinable program, the join stage returns a conjunction with the same logical consequences. 
Proposition \ref{lem_join} shows that given all joinable programs, the join stage returns all non-subsumed splittable combinable programs.
% Proposition \ref{lem_join} shows that given all non-splittable non-separable programs, the join stage returns all non-subsumed non-separable combinable programs \ac{NEW}.
Therefore, \name{} builds all non-subsumed splittable and non-splittable combinable programs.
% non-subsumed combinable programs.
% there are finitely many splittable combinable programs and that the join stage can build them all \ac{from a quick read, is this true?}
% Given the set of all combinable programs, the combine stage returns a solution \cite{combo}.
% By Assumption \ref{existencesol}, a solution exists.
By Proposition \ref{prop_combine}, given all non-subsumed combinable programs, the combine stage returns an optimal solution.
Therefore, \name{} without the constrain stage returns an optimal solution.
\end{proof}

\noindent
We show the correctness of the \name{}:
\begin{theorem}[\textbf{Correctness of \name{}}]
\name{} returns an optimal solution.
\end{theorem}
\begin{proof}
From Proposition \ref{correctness}, \name{} without the constrain stage returns an optimal solution.
% \ac{can return every solution}.
From Proposition \ref{prop_opt_sound}, the constrain stage never prunes an optimal solution. 
Therefore, \name{} with the constrain stage returns an optimal solution.
% Moreover, \name{} uses iterative deepening over the program size to guarantee optimality. Therefore \name{} returns an optimal solution.
% \ac{From prop X, joiner without constraints always returns an optimal solution.
% From prop X, the constraint stage never prunes an optimal solution.
% Therefore, joiner with the constrain stage always returns an optimal solution.}
\end{proof}




